$O(n \log n)$-time text compression by LZ-style longest first substitution

Mauer et al. [A Lempel-Ziv-style Compression Method for Repetitive Texts, PSC 2017] proposed a hybrid text compression method called LZ-LFS which has both features of Lempel-Ziv 77 factorization and longest first substitution. They showed that LZ-LFS can achieve better compression ratio for repetitive texts, compared to some state-of-the-art compression algorithms. The drawback of Mauer et al.'s method is that their LZ-LFS compression algorithm takes $O(n^2)$ time on an input string of length $n$. In this paper, we show a faster LZ-LFS compression algorithm that works in $O(n \log n)$ time. We also propose a simpler version of LZ-LFS that can be computed in $O(n)$ time.

==> parameters.tex <==
\section{On parameters $\alpha$ and $\beta$}

The algorithm of Mauer et al.~\cite{MauerBO17}
uses the suffix array and the LCP array~\cite{manber93:_suffix}
of the input string $w$,
and finds an LR $x_k$ for $w_k$ at each $k$-th step
using a maximal interval of the LCP array.

The suffix array $\SA$ for a string $w$ of length $n$ is a permutation
of $[1..n]$ such that $\SA[j] = i$ iff
$w[i..]$ is the lexicographically $j$-th suffix of $w$.
The LCP array $\LCP$ for $w$ is an array of length $n$
such that $\LCP[1] = 0$ and 
$\LCP[i]$ stores the length
of the longest common prefix of $w[\SA[i-1]..]$ and $w[\SA[i]..]$
for $2 \leq i \leq n$.

An interval $[i..j]$ of $\LCP$ array of $w$
is called a \emph{$p$-interval} if
(1) $\LCP[i-1] < p$ or $i = 1$,
(2) $\LCP[k] \geq p$ for all $i \leq k \leq j$,
(3) $\LCP[k] = p$ for some $i \leq k \leq j$, and
(4) $\LCP[j+1] < p$ or $j = n$.
An interval $[i..j]$ of $\LCP$ array of $w$
is called a \emph{maximal interval} if
it is a $p$-interval for some $p \geq 1$
and the longest common prefix of length $p$
for all the corresponding suffixes $w[\SA[i]..], \ldots, w[\SA[j]..]$ 
is a maximal repeat of $w$.
Mauer et al.'s algorithm picks up maximal intervals
as candidates for LRs to replace.

Let $\bit(w')$, $\bit(F)$, and $\bit(\Factors)$ respectively denote
the average number of bits to encode a single character from $w'$,
an element of $F$, and an element of $\Factors$ with a fixed encoding scheme.
The original algorithm by Mauer et al.~\cite{MauerBO17}
uses two parameters $\alpha$ and $\beta$ such that
$\alpha = \frac{\bit(\Factors)}{\bit(w')}$ and
$\beta = 1 + \frac{\bit(F)}{\bit(w')}$.
In each $k$-th step, their algorithm performs
replacement of an LR $x_k$ of length $\len_k$
only if the following conditions holds:
\begin{equation}
  \len_k \geq \frac{\alpha}{s} + \beta,
  \label{eqn:alpha_beta}
\end{equation}
where $s$ denotes the number of Type 2 and Type 3 occurrences
of the LR $x_k$ in the current string $w_k$.
However, since the values of $\alpha$ and $\beta$ cannot be precomputed,
in their implementation of LZ-LFS,
they use ad-hoc pre-determined values for $\alpha$ and $\beta$
(see~\cite{MauerBO17} for details).

However, we have found that there exist a series of strings
and settings of $\alpha$ and $\beta$
for which Mauer et al.'s algorithm fails to recursively replace LRs.

Consider a series of strings
\[
w = aXabaXaXac\$,
\]
where $a, b, c \in \Sigma$ and $X \in (\Sigma \setminus \{a, b, c\})^+$.
This string $w = w_1$ has a unique LR $aXa$.
Since there are three occurrences of $aXa$ in $w$
and the second and third occurrences overlap,
the second occurrence is of Type 2.
Hence, we have $s = 1$ and $\len_1 = k+2$,
where $k = |X|$.
Then, if the pre-determined values of $\alpha$ and $\beta$
satisfy $\alpha = k+2$ and $\beta = k/2$,
Equation~(\ref{eqn:alpha_beta}) does not hold.
Hence, the original algorithm of Mauer et al. does not
replace $aXa$ and tries to find a next LR (which can be shorter than $aXa$).
In this case, the second longest repeats are
$aX$ and $Xa$ of length $k+1$ each.
However, since neither is $aX$ nor $Xa$ a maximal repeat,
it is not represented by a maximal interval of the LCP array.
Hence, neither is $aX$ nor $Xa$ selected for replacement.
Moreover, note that even $X$ is not a maximal repeat,
and that there are no repeats of length at least two
consisting only of $a$, $b$, and/or $c$.
Therefore, Mauer et al.'s algorithm terminates at this point.

Note that one can easily construct even worse instances
where more candidates of LRs have to be skipped,
by adding other strings from $(\Sigma \setminus \{a, b, c\})^* \setminus \{X\}$
to the input string in a similar manner to the occurrences of $X$.

Given the above observation,
in our algorithm that follows,
we will omit the condition of Equation~\ref{eqn:alpha_beta},
and will replace the Type 1, 2, 3 occurrences of \emph{any} selected LR.




